$\mu$SE: Mutation-based Evaluation of Security-focused Static Analysis Tools for Android

This demo paper presents the technical details and usage scenarios of $\mu$SE: a mutation-based tool for evaluating security-focused static analysis tools for Android. Mutation testing is generally used by software practitioners to assess the robustness of a given test-suite. However, we leverage this technique to systematically evaluate static analysis tools and uncover and document soundness issues. $\mu$SE's analysis has found 25 previously undocumented flaws in static data leak detection tools for Android. $\mu$SE offers four mutation schemes, namely Reachability, Complex-reachability, TaintSink, and ScopeSink, which determine the locations of seeded mutants. Furthermore, the user can extend $\mu$SE by customizing the API calls targeted by the mutation analysis. $\mu$SE is also practical, as it makes use of filtering techniques based on compilation and execution criteria that reduces the number of ineffective mutations.

==> img/__latexindent_temp.tex <==
\begin{figure*}[htbp]
    \begin{center}

      \includegraphics[width=.7\textwidth]{img/design}
    \end{center}
      \caption{\small The components and process of the \tool{}.}\label{fig:design}
\end{figure*}

==> img/default_img.tex <==
\begin{figure}[htbp]
    \centerline{\includegraphics{fig1.png}}
    \caption{Example of a figure caption.}
    \label{fig:design}
\end{figure}


==> table/default_table.tex <==
\begin{table}[htbp]
    \caption{Table Type Styles}
    \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
    \cline{2-4}
    \textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
    \hline
    copy& More table copy$^{\mathrm{a}}$& &  \\
    \hline
    \multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
    \end{tabular}
    \label{tab1}
    \end{center}
    \end{table}

==> table/table_leak_executable.tex <==
\begin{table}[t]
    \caption{
        % {\color{blue}
        The number of leaks inserted by \tool, and the final number marked as executable by \tools EE{}. Note that the ``-'' indicates that the scheme is not applicable to a particular app, due to the app's particular characteristics (\eg, the absence of fragments)
        % }
        }
    % \vspace{-0.5em}
    \scriptsize
    \centering
    \begin{tabular*}{.5\textwidth}{l @{\extracolsep{\fill}} l l l l}
        \toprule
        \textbf{App} & \textbf{Reachability} & \textbf{ScopeSink} & \textbf{TaintSink} & \textbf{\begin{tabular}[c]{@{}l@{}}Complex \\ Reachability\end{tabular}}
\\
        % \cmidrule(r){1-1}\cmidrule(lr){2-5}\cmidrule(lr){6-9}
        \midrule
        2048  & 24  & 48   & 66     & 22   \\
        % & 13  ($\approx$54\%)  & 12  ($\approx$12\%)   & 8    ($\approx$12\%) & 11   ($\approx$50\%)\\

        Protect Baby Monitor  & 106  & -   & 231    & 83   \\
        % & 63  ($\approx$59\%)  & -                     & 80   ($\approx$34\%) & 44   ($\approx$14\%)\\

        QR Scanner  & 248  & -    & 668   & 191  \\
        % & 51  ($\approx$20\%)  & -                     & 162  ($\approx$24\%) & 36   ($\approx$26\%)\\
        Location Share  & 45   & 192  & 346   & 41   \\
        % & 20  ($\approx$44\%)  & 156 ($\approx$81\%)   & 51   ($\approx$14\%) & 23   ($\approx$2\%)\\
        Camera Roll & 3181 & -    & 12104 & 2777 \\
        % & 598 ($\approx$18\%)  & -                     & 1362 ($\approx$11\%) & 508  ($\approx$42\%)\\
        AndroidPN Client  & 434  & -    & 2699  & 384  \\
        % & 57  ($\approx$13\%)  & -                     & 110  ($\approx$4\%)  & 51   ($\approx$5\%)\\
        Activity Launcher & 204  & -    & 551   & 174  \\
        % & 111 ($\approx$54\%)  & -                     & 243  ($\approx$44\%) & 95   ($\approx$34\%)\\
        Man Man  & 975  & 1193 & 5266  & 839  \\
        % & 215 ($\approx$22\%)  & 56  ($\approx$4\%)    & 567  ($\approx$10\%) & 168  ($\approx$32\%)\\
        BMI Calculator  & 23   & 8    & 20    & 21   \\
        % & 15 ($\approx$65\%)  & 6   ($\approx$75\%)   & 13   ($\approx$65\%) & 12   ($\approx$7\%)\\
        Time Tracker  & 476  & -    & 5283  & 449  \\
        % & 59($\approx$12\%)  & -                     & 681  ($\approx$12\%) & 54   ($\approx$11\%)\\
        AFH Downloader  & 316  & 1111 & 827   & 277  \\
        % & 50   ($\approx$15\%)  & 287 ($\approx$25\%)   & 83   ($\approx$10\%) & 41   ($\approx$5\%)\\
        Android Explorer  & 250  & 354  & 428   & 213\\
        %   & 77  ($\approx$30\%)  & 111 ($\approx$31\%)   & 59   ($\approx$13\%) & 38   ($\approx$7\%)\\
        Kaltura Device Info  & 156  & 203  & 828   & 147  \\
        % & 89  ($\approx$57\%)  & 112 ($\approx$55\%)   & 295  ($\approx$35\%) & 84   ($\approx$71\%)\\
        Apod Classic  & 125  & 844  & 663   & 107  \\
        % & 79  ($\approx$63\%)  & 55  ($\approx$6\%)    & 27   ($\approx$4\%)  & 59   ($\approx$9\%)\\
        CalendarTrigger & 1304 & 3478 & 2790  & 1143 \\
        % & 211 ($\approx$16\%)  & 456 ($\approx$13\%)   & 172  ($\approx$6\%)  & 154  ($\approx$41\%)\\
        % \midrule
        % \textbf{Total}  & 7867 & 7431 & 32770 & 6868 & 1708 ($\approx$22\%) & 1251 ($\approx$16\%) & 3913 ($\approx$11\%) & 1378 ($\approx$20\%) \\
    \bottomrule\label{tbl:leaks_inserted_executable}
    \end{tabular*}
    % \vspace{-1.5em}
\end{table}

==> tex/conclusion.backup.tex <==
\section{Conclusion}
In this demonstration paper, we discussed the technical approach, implementation and usage details of mutation based soundness evaluation framework, namely  \tool{}. Our approach helps detect soundness issues in SASTs

==> tex/demonstration.backup.tex <==
\section{Usage}
\input{img/screenshot.tex}
\input{listing/configuration.tex}
\tool{} can be used through both Command Line Interface (CLI) and Graphical User Interface (GUI).
This allows \tool{} to be used as both standalone software as well as component of other software.
\tool{} relies on Java LTS 11.0 for compilation and runtime.
In addition, the GUI depends on OpenJFX version 11.0.2.
Furthermore, a \texttt{JAVA\_HOME} is required to be declared in environment variable as it is required for checking compilation issues.

To get started with mutation either through CLI or GUI - a configuration file as shown in Listing~\ref{lst:configuration} is required which specifies:
\begin{itemize}
    \item \textbf{lib4ast path} - contains definition libraries required for AST, such as \texttt{android.jar}
    \item \textbf{Mutation Scheme} - Choice of mutation scheme, currently available choices are Reachability, Complex-Reachability, TaintSink, and ScopeSink
    \item \textbf{App source Location} - Path of project that is to be mutated
    \item \textbf{Destination Path} - Path where mutated project will be saved
    \item \textbf{App Name} - Name of the project
\end{itemize}

By default, \tool{} uses Android and Java specific API (\texttt{android.util.Log} and \texttt{java.util.Calendar}) for creating source and sink related calls.
However, this can be customized by user by specifying the variable format and involved APIs in a configuration file as shown in Listing~\ref{lst:configuration}.
\input{listing/cliuse.tex}
Because of the configuration file, using \tool{} is simple - only the path to configuration file is required a parameter for the CLI as shown in Listing~\ref{lst:cli_use}.
On the other hand, user can also use the GUI as shown in Figure~\ref{fig:screenshot} which will walk the user through different configuration settings, helping the user to save/load a configuration file for use.
\input{listing/output.tex}
When \tool{} is executed, it creates mutants while creating logs as shown in Listing~\ref{lst:output}.


==> tex/related_work.tex <==
\section{Related Work}
related work
